Reasons and Means to Model Preferences as Incomplete

Literature involving preferences of artificial agents or human beings often assume their preferences can be represented using a complete transitive binary relation. Much has been written however on different models of preferences. We review some of the reasons that have been put forward to justify more complex modeling, and review some of the techniques that have been proposed to obtain models of such preferences.

==> preamble/refAPIcmds.tex <==
\newbool{refAPIIsAnnotation}
\newbool{refAPIDisplayFull}
\pgfkeys{
	/refAPI/.is family,
	/refAPI/.cd,
	base url/.estore in = \refAPIBaseUrl,
	@/.is if = refAPIIsAnnotation,
	full/.is if = refAPIDisplayFull,
	prefix/.store in = \refAPIPrefix,
	suffix/.estore in = \refAPISuffix,
	default/.style = {
		base url = ,
		@ = false,
		full = false,
		prefix = \texttt,
		suffix = ,
	},
}

%Usage: \refAPIParseRef{javax.persistence/EntityManager} ; \refAPIParseRef{javax.persistence/PersistenceContextType\#EXTENDED}
%Defines: \refAPIFQName (before #) ; \refAPIField (after #) ; \refAPIPackageSlashes (FQName before / with slashes instead of dots) ; \refAPIClass (FQName after /)
\newcommand{\refAPIParseRef}[1]{%
	\IfSubStr{#1}{\#}{%
		\StrBefore{#1}{\#}[\refAPIFQName]%
		\StrBehind{#1}{\#}[\refAPIField]%
	}{%
		\edef\refAPIFQName{#1}%
		\edef\refAPIField{}%
	}%
	\StrBefore{\refAPIFQName}{/}[\refAPIPackage]%
	\StrBehind{\refAPIFQName}{/}[\refAPIClass]%
	\StrSubstitute{\refAPIPackage}{.}{/}[\refAPIPackageSlashes]%
}

%Usage: \jeeref{javax.persistence/EntityManager} ; \jeeref[@]{javax.persistence/PersistenceContextType\#EXTENDED}
\newcommand{\jeeref}[2][]{\refAPIParseRef{#2}\jrefAPI{base url = https://docs.oracle.com/javaee/7/api/, #1}}
\newcommand{\jseref}[2][]{\refAPIParseRef{#2}\jrefAPI{base url = https://docs.oracle.com/javase/8/docs/api/, #1}}
\newcommand{\jsftag}[2][]{\refAPIParseRef{#2}\jrefAPI{base url = https://docs.oracle.com/javaee/7/javaserver-faces-2-2/vdldocs-facelets/, full, prefix=:, #1}}
%Standard HTML RenderKit : https://docs.oracle.com/javaee/7/javaserver-faces-2-2/renderkitdocs/HTML_BASIC/javax.faces.Inputjavax.faces.Text.html

%Accepts keys: @, prefix, suffix. Requires key: base url. Expects defined: \refAPIField ; \refAPIPackageSlashes ; \refAPIClass
\newcommand{\jrefAPI}[1]{%
	\pgfkeys{/refAPI/.cd, default, #1}%
	\ifbool{refAPIIsAnnotation}{%
		\edef\refAPIAnnot{@}%
	}{%
		\edef\refAPIAnnot{}%
	}%
	\IfEq{\refAPIField}{}{%
		{%
			\ifbool{refAPIDisplayFull}{%
				\refAPIPackage%
			}{%
			}%
			\refAPIPrefix{%
			\href{%
				\refAPIBaseUrl\refAPIPackageSlashes/\refAPIClass.html\#\refAPIField%
			}{%
				\refAPIAnnot\refAPIClass%
			}%
		}\refAPISuffix}%
	}{%
		{\refAPIPrefix{%
			\refAPIAnnot\refAPIClass.%
			\href{%
				\refAPIBaseUrl\refAPIPackageSlashes/\refAPIClass.html%
			}{%
				\refAPIField%
			}%
		}\refAPISuffix}%
	}%
}



==> preamble/uml.tex <==
%this approach does not generalize to multipart nodes.
%\tikzset{/uml/interface/.style={rectangle, draw, fill=yellow!20, align=left, node font=\fontspec{Latin Modern Mono Light}, node contents={$<<$interface$>>$\\\textbf{#1}}, name=#1
%}}
%this approach does not apply for <<interface>>. Never mind, I’ll do it manually, as I can’t find anything better. Use: \nodepart[font=]{one} \small <<interface>>\\\bfseries ItemDAO
\tikzset{/uml/class/.style={rectangle, draw, align=center, fill=yellow!20, node font=\fontspec{Latin Modern Mono Light}, font=\bfseries
}}
\tikzset{/uml/abstract class/.style={rectangle, draw, align=center, fill=yellow!20, node font=\fontspec{Latin Modern Mono Light}, font=\bfseries\itshape
}}
\tikzset{/uml/class3/.style={
rectangle split, rectangle split every empty part={}, rectangle split parts=3, rectangle split part align={center, left, left}, draw, fill=yellow!20, rectangle split empty part height=0, node font=\fontspec{Latin Modern Mono Light}, every one node part/.style={font=\bfseries, align=center}, every two node part/.style={align=left}, every three node part/.style={align=left}
}}
\tikzset{/uml/extends/.style={draw, -open triangle 45}}
\tikzset{/uml/implements/.style={draw, -open triangle 45, dashed}}
%prefix= used to cancel \texttt, otherwise this cancels the effect of the font selection \fontspec{Latin Modern Mono Light}, and thus renders \bfseries inoperant. With prefix=, the result is correct.
%\jeeref[prefix=]{javax.faces.component.html/HtmlCommandButton}\\
\tikzset{/uml/table/.style={rectangle, draw, align=center, fill=blue!20, node font=\fontspec{Latin Modern Mono Light}, font=\bfseries
}}
\tikzset{/uml/table2/.style={
rectangle split, rectangle split every empty part={}, rectangle split parts=2, rectangle split part align={center, left}, draw, fill=blue!20, rectangle split empty part height=0, node font=\fontspec{Latin Modern Mono Light}, every one node part/.style={font=\bfseries, align=center}, every two node part/.style={align=left}
}}
\tikzset{/uml/dbkey/.style={draw, ->}}
%http://tex.stackexchange.com/questions/79781/placing-anchor-before-and-after-text-in-multipart-rectangle


